Software-defined Dynamic 5G Network Slice Management for Industrial Internet of Things

This paper addresses the challenges of delivering fine-grained Quality of Service (QoS) and communication determinism over 5G wireless networks for real-time and autonomous needs of Industrial Internet of Things (IIoT) applications while effectively sharing network resources. Specifically, this work presents DANSM, a software-defined, dynamic and autonomous network slice management middleware for 5G-based IIoT use cases, such as adaptive robotic repair. Empirical studies evaluating DANSM on our testbed comprising a Free5GC-based core and UERANSIM-based simulations reveal that the software-defined DANSM solution can efficiently balance the traffic load in the data plane thereby reducing the end-to-end response time and improve the service performance by completing 34% more subtasks than a Modified Greedy Algorithm (MGA), 64% more subtasks than First Fit Descending (FFD) and 22% more subtasks than Best Fit Descending (BFD) approaches all while minimizing operational costs.

==> acknowledgment.tex <==
\section*{Acknowledgment}
\label{sec:Acknowledgment}
This work is supported in part by funding from Siemens Technology. Any
opinions, findings, and conclusions or recommendations expressed in this
material are of the author(s) and do not necessarily reflect the views of the
sponsor. 


==> algorithm.tex <==
% \begin{algorithm}[]
%  \caption{Heuristic Scheduling Algorithm} \label{MG}
%  \KwIn{A Directed Acyclic Graph(DAG) $D$ of tasks, a UE arrivel time list T, an empty UE waitlist $UE_waitlist$, the objective function Eq.(9) $F(x)$ formulated from queueing model}.
 
%     \SetKwFunction{FMain}{Check\_UE\_Status}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Fn{\FMain{$U$, $\lambda$, $L$}}{
%         $UE_{waitlist} = [ ]$\;
%          \For{$i\gets1$ \KwTo $n$}{
            
%             \If{$u_{i}$ changed repairing task}{
%                 % $p_{ui} \leftarrow P\_Function(u_{i},\lambda_{i},l_{i})$\;
%                 add $(u_{i},\lambda_{i},l_{i})$ to $UE_{waitlist}$ \; 
%           }
%          }
        
%         \Return {$UE_{waitlist}$} \;
%      }
%     \textbf{End Function}
    
%     \SetKwFunction{FMain}{Main}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Fn{\FMain{$UPFs$, $m$, $U$, $n$, $\Lambda$, $\Theta$, $X_{0}$, $MF$}}{
       
%         \While{$MF$}{
%             $UE_{waitlist} \leftarrow$ \Call{Check\_UE\_Status}{$U$, $\lambda$, $L$}\;
%             \If{ $UE_{waitlist}$ is not empty}{
%             Sort $UE_{waitlist}$ based on the job priority and the job start time\; 
%             % Sort $\Theta$ in descending order based on the existing loads of all network slicing\; 
%             \For{$j\gets1$ \KwTo length ($UE_{waitlist}$)}{
%                 Assign $u_{j}$ to the matched network slicing in $S$\;
%                 \For{$p\gets1$ \KwTo length ($UPFs$)}{
%                     \If{}                
%                 }
%                 }
%             }
            
%         }
%         \Return {$X_{0}$}\;
%     }
%      \textbf{End Function}
    
% \end{algorithm}
